Registered Attribute-Based Encryption with Publicly Verifiable Certified Deletion, Everlasting Security, and More

Certified deletion ensures that encrypted data can be irreversibly deleted, preventing future recovery even if decryption keys are later exposed. Although existing works have achieved certified deletion across various cryptographic primitives, they rely on central authorities, leading to inherent escrow vulnerabilities. This raises the question of whether certified deletion can be achieved in decentralized frameworks such as Registered Attribute-Based Encryption (RABE) that combines fine-grained access control with user-controlled key registration. This paper presents the first RABE schemes supporting certified deletion and certified everlasting security. Specifically, we obtain the following: - We first design a privately verifiable RABE with Certified Deletion (RABE-CD) scheme by combining our newly proposed shadow registered ABE (Shad-RABE) with one-time symmetric key encryption with certified deletion. - We then construct a publicly verifiable RABE-CD scheme using Shad-RABE, witness encryption, and one-shot signatures, allowing any party to validate deletion certificates without accessing secret keys. - We also extend to privately verifiable RABE with Certified Everlasting Deletion (RABE-CED) scheme, integrating quantum-secure RABE with the certified everlasting lemma. Once a certificate is produced, message privacy becomes information-theoretic even against unbounded adversaries. -We finally realize a publicly verifiable RABE-CED scheme by employing digital signatures for the BB84 states, allowing universal verification while ensuring that deletion irreversibly destroys information relevant to decryption.

==> 4_Syntax-RABE-CD-V2.tex <==
\section{\textsf{RABE} with Certified Deletion}\label{section:RABE-CD}
In this section, we first introduce the system model of the registered attribute-based encryption with certified deletion (\textsf{RABE-CD}) protocol along with its correctness and security properties. We then present generic constructions of \textsf{RABE-CD} protocol under two verification paradigms: one supporting private verification of deletion and the other enabling public verification. Finally, we provide the lattice-based instantiations of \textsf{RABE-CD} protocols in both private verification and public verification settings.%\vspace{0.2cm}

%\noindent\textbf{Syntax of \textsf{RABE-CD}.}
\subsection{System Model of \textsf{RABE-CD}}\label{def:RABE-CD}
%----------------------------------- 
Let $\lambda$ be the security parameter. Let $\mathcal{U} = \{\mathcal{U}_\lambda\}_{\lambda \in \mathbb{N}}$ denotes the attribute universe, $\mathcal{P} = \{\mathcal{P}_\lambda\}_{\lambda \in \mathbb{N}}$ represents the policy space, and $\mathcal{M} = \{\mathcal{M}_\lambda\}_{\lambda \in \mathbb{N}}$ stands the message space. A \textsf{RABE-CD} scheme consists of the tuple of efficient algorithms $\prod^{\mathsf{RABE}}_{\textsf{CD}} =$ $(\mathsf{Setup},$ $\mathsf{KeyGen},$ $\mathsf{RegPK},$ $\mathsf{Encrypt},$ $\mathsf{Update},$ $\mathsf{Decrypt},$ $\mathsf{Delete},$ $\mathsf{Verify})$ with the following syntax:\vspace{0.2cm}

\begin{description}\setlength\itemsep{0.5em}
%----------------------------
\item[$-$] $(\textsf{crs}) \leftarrow \textsf{Setup}(1^{\lambda}, 1^{|\mathcal{U}|}).$  
On the input of the length of the security parameter $\lambda$ and the size of the attribute universe $\mathcal{U}$, the setup algorithm outputs a common reference string $\mathsf{crs}$.
%----------------------------
\item[$-$] {(\textsf{pk}, \textsf{sk})} $\leftarrow \mathsf{KeyGen}(\mathsf{crs}, \mathsf{aux}, P).$  
Given the common reference string \textsf{crs}, an auxiliary state $\mathsf{aux}$ (possibly empty) and a policy $P\in \mathcal{P}$, the key generation algorithm outputs a public key $\mathsf{pk}$ and secret key $\mathsf{sk}$.
%----------------------------
\item[$-$] $(\mathsf{mpk}, \mathsf{aux}') \leftarrow \mathsf{RegPK}(\mathsf{crs}, \mathsf{aux}, \mathsf{pk}, P).$  The registration algorithm takes as input a common reference string \textsf{crs}, an auxiliary state \textsf{aux}, and a public key $\mathsf{pk}$, and a policy $P\in \mathcal{P}$ to return an updated master public key $\mathsf{mpk}$ and auxiliary state $\mathsf{aux}'$.
%---------------------------
\item[$-$] $(\mathsf{vk}, \mathsf{ct}) \leftarrow \mathsf{Encrypt}\left( \mathsf{mpk}, X, \mu \right).$ The encryption algorithm takes as input the master public key $\mathsf{mpk}$, an \textcolor{orange}{ attribute $X \in \mathcal{U_{\tau}}$}, and a message $\mu$ to produce a verification key $\mathsf{vk}$ together with a ciphertext $\mathsf{ct}$.

%---------------------------
\item[$-$] $(\mathsf{hsk}) \leftarrow \mathsf{Update}(\mathsf{crs}, \mathsf{aux}, \mathsf{pk}).$ Taking as input the common reference string \textsf{crs}, a auxiliary state \textsf{aux}, and a public key \textsf{pk}, the update algorithm deterministically outputs a helper decryption key $\mathsf{hsk}$.
%---------------------------
\item[$-$] $(\mu \cup \{\perp, \mathsf{GetUpdate}\}) \leftarrow \mathsf{Decrypt}(\mathsf{sk}, \mathsf{hsk}, \mathsf{ct}).$ On input of the secret key \textsf{sk}, a helper key \textsf{hsk}, and a ciphertext \textsf{ct}, the decryption algorithm outputs the message $\mu$, a failure symbol $\perp$, or the flag $\mathsf{GetUpdate}$ indicating that an updated helper key is needed.
%---------------------------
\item[$-$] $(\mathsf{cert}) \leftarrow \mathsf{Delete}(\mathsf{ct}).$  
The deletion algorithm generates a deletion certificate $\mathsf{cert}$ for the given ciphertext \textsf{cert}.
%---------------------------
\item[$-$] $(b) \leftarrow \mathsf{Verify}(\mathsf{vk}, \mathsf{cert}).$  
Given a verification key \textsf{vk} and a deletion certificate \textsf{cert}, the verification algorithm outputs $1$ if valid, $0$ otherwise. This check is publicly executable.
\end{description}
%--------------------------------------------
 
% \noindent\textbf{Correctness and Efficiency of \textsf{RABE-CD}.}\label{def:rabe-cd-correctness} 
\subsection{Correctness and Efficiency of \textsf{RABE-CD}}\label{def:rabe-cd-correctness}
Let $\prod^{\mathsf{RABE}}_{\textsf{CD}}$ denote a registered attribute-based encryption scheme with certified deletion protocol defined over an attribute universe $\mathcal{U}$, a policy space $\mathcal{P}$, and a message space $\mathcal{M}$. To define the correctness of $\prod^{\mathsf{RABE}}_{\textsf{CD}}$, we specify two experiments, Decryption Game and Verification Game, played between an adversary $\mathcal{A}$ and a challenger.\vspace{0.2cm}

\begin{description}\setlength\itemsep{0.5em}
    \item[$\bullet$] \textbf{Setup phase:} The challenger starts by sampling the common reference string $\mathsf{crs} \leftarrow \mathsf{Setup}(1^\lambda, 1^{|\mathcal{U}|})$. It then initializes the auxiliary input as $\mathsf{aux} \leftarrow \bot$ and sets the initial master public key to $\mathsf{mpk}_0 \leftarrow \bot$. Next, it initializes a counter $\mathsf{ctr}_{\mathsf{reg}} \leftarrow 0$ to record the number of registration queries and another counter $\mathsf{ctr}_{\mathsf{enc}} \leftarrow 0$ to track the number of encryption queries. In addition, it sets $\mathsf{ctr}^\ast_{\mathsf{reg}} \leftarrow \infty$ as the index of the target key, which may be updated during the game. Finally, the challenger sends $\mathsf{crs}$ to $\mathcal{A}$.
    
    \item[$\bullet$] \textbf{Query phase:} The adversary $\mathcal{A}$ may adaptively issue the following queries.\vspace{0.2cm}
    
    \begin{description}\setlength\itemsep{0.5em}
        \item[$-$] \textbf{Register non-target key query:} In this query, $\mathcal{A}$ provides a public key $\mathsf{pk}$ and a set of attributes $S \subseteq \mathcal{U}$. The challenger first increments the counter $\mathsf{ctr}_{\mathsf{reg}} \gets \mathsf{ctr}_{\mathsf{reg}} + 1$, then registers the key by computing $(\mathsf{mpk}_{\mathsf{ctr}_{\mathsf{reg}}}, \mathsf{aux}') \gets \mathsf{RegPK}(\mathsf{crs}, \mathsf{aux}, \mathsf{pk}, S)$. It updates the auxiliary data by setting $\mathsf{aux} \gets \mathsf{aux}'$, and replies to $\mathcal{A}$ with $(\mathsf{ctr}_{\mathsf{reg}}, \mathsf{mpk}_{\mathsf{ctr}_{\mathsf{reg}}}, \mathsf{aux})$.
        
        \item[$-$] \textbf{Register target key query:} In the register target key query, $\mathcal{A}$ specifies a target set of attributes $S^\ast \subseteq \mathcal{U}$. If a target key has already been registered, the challenger replies with $\bot$. Otherwise, it increments the counter $\mathsf{ctr}_{\mathsf{reg}} \gets \mathsf{ctr}_{\mathsf{reg}} + 1$, samples $(\mathsf{pk}^\ast, \mathsf{sk}^\ast) \gets \mathsf{KeyGen}(1^\lambda)$, and registers the key by computing $(\mathsf{mpk}_{\mathsf{ctr}_{\mathsf{reg}}}, \mathsf{aux}') \gets \mathsf{RegPK}(\mathsf{crs}, \mathsf{aux}, \mathsf{pk}^\ast, S^\ast)$. It then computes the helper decryption key $\mathsf{hsk}^\ast \gets \mathsf{Update}(\mathsf{crs}, \mathsf{aux}, \mathsf{pk}^\ast)$, updates $\mathsf{aux} \gets \mathsf{aux}'$, and records the index of the target key as $\mathsf{ctr}^\ast_{\mathsf{reg}} \gets \mathsf{ctr}_{\mathsf{reg}}$. Finally, it replies to $\mathcal{A}$ with $(\mathsf{ctr}_{\mathsf{reg}}, \mathsf{mpk}_{\mathsf{ctr}_{\mathsf{reg}}}, \mathsf{aux}, \mathsf{pk}^\ast, \mathsf{hsk}^\ast, \mathsf{sk}^\ast)$.

        \item[$-$] \textbf{Encryption query:} In an encryption query, $\mathcal{A}$ provides an index $\mathsf{ctr}^\ast_{\mathsf{reg}} \leq i \leq \mathsf{ctr}_{\mathsf{reg}}$, a message $\mu_{\mathsf{ctr}_{\mathsf{enc}}} \in \mathcal{M}$, and a policy $P_{\mathsf{ctr}_{\mathsf{enc}}} \in \mathcal{P}$. If no target key has been registered, or if the target set of attributes $S^\ast$ does not satisfy $P_{\mathsf{ctr}_{\mathsf{enc}}}$, the challenger replies with $\bot$. Otherwise, it increments $\mathsf{ctr}_{\mathsf{enc}} \gets \mathsf{ctr}_{\mathsf{enc}} + 1$ and computes $\mathsf{ct}_{\mathsf{ctr}_{\mathsf{enc}}} \gets \mathsf{Encrypt}(\mathsf{mpk}_i, P_{\mathsf{ctr}_{\mathsf{enc}}}, \mu_{\mathsf{ctr}_{\mathsf{enc}}})$. The challenger then replies with $(\mathsf{ctr}_{\mathsf{enc}}, \mathsf{ct}_{\mathsf{ctr}_{\mathsf{enc}}})$.

        \item[$-$] \textbf{Decryption query:}  In a decryption query, the adversary submits a ciphertext index $1 \leq j \leq \mathsf{ctr}_{\mathsf{enc}}$. The challenger computes $m'_j \gets$ $\mathsf{Decrypt}(\mathsf{sk}^\ast,$ $\mathsf{hsk}^\ast,$ $\mathsf{ct}_j)$. If $m'_j = \mathsf{GetUpdate}$, it updates $\mathsf{hsk}^\ast \gets \mathsf{Update}(\mathsf{crs}, \mathsf{aux}, \mathsf{pk}^\ast)$ and recomputes $m'_j \gets \mathsf{Decrypt}(\mathsf{sk}^\ast, \mathsf{hsk}^\ast, \mathsf{ct}_j)$. If $m'_j \neq \mu_j$, the experiment halts with output $b=0$ (Decryption Game).

        \item[$-$] \textbf{Verification query:} In a verification query, the adversary submits a ciphertext index $j$. The challenger computes $\mathsf{cert}_j \gets \mathsf{Delete}(\mathsf{ct}_j)$ and $v_j \gets \mathsf{Verify}(\mathsf{vk}_j, \mathsf{cert}_j)$. If $v_j \neq 1$, the experiment halts with output $b=0$ (Verification Game).
    \end{description}
    If the adversary finishes making queries without halting the Decryption Game, the experiment outputs $b=1$. Similarly, if the Verification Game does not halt, the output is $b=1$.
\end{description}

\noindent We say that the scheme $\prod^{\mathsf{RABE}}_{\textsf{CD}}$ is correct and efficient if for all (possibly unbounded) $\mathcal{A}$ making at most polynomially many queries, the following hold:
\begin{description}\setlength\itemsep{0.5em}
    \item[$\bullet$] \textbf{Decryption correctness:} There exist a negligible function $\mathsf{negl}$ in $\lambda$ such that $\Pr[b = 0] = \mathsf{negl}(\lambda)$ in the Decryption Game.

    \item[$\bullet$] \textbf{Verification correctness:} There exists a negligible function $\mathsf{negl}$ in $\lambda$ such that $\Pr[b = 0] = \mathsf{negl}(\lambda)$ in the Verification Game.

    \item[$\bullet$] \textbf{Compactness:} Let $N$ be the number of registration queries. There exists a polynomial $\mathsf{poly}$ such that for all $i\in[N]$,
    \[
        |\mathsf{mpk}_i| = \mathsf{poly}(\lambda, |\mathcal{U}|, \log i), \quad
        |\mathsf{hsk}^\ast| = \mathsf{poly}(\lambda, |\mathcal{U}|, \log N).
    \]

    \item[$\bullet$] \textbf{Update efficiency:} Let $N$ denote the number of registration queries issued by $\mathcal{A}$ in the above game. During the game, the challenger invokes $\mathsf{Update}$ at most $\mathcal{O}(\log N)$ times, and each invocation runs in $\mathsf{poly}(\log N)$ time in the \textsf{RAM} model. In particular, we model $\mathsf{Update}$ as a \textsf{RAM} program with random access to its input, then its running time may be smaller than the input length.
\end{description}\vspace{0.2cm}
%----------------------------------

% \noindent\textbf{Certified Deletion Security of \textsf{RABE-CD}.}\label{Security-def:RABE-CD}
\subsection{Certified Deletion Security of \textsf{RABE-CD}}\label{Security-def:RABE-CD}
Let $\prod^{\mathsf{RABE}}_{\textsf{CD}}$ denote a registered attribute-based encryption with certified deletion protocol defined over an attribute universe $\mathcal{U}$, a policy space $\mathcal{P}$, and a message space $\mathcal{M}$. For a security parameter $\lambda$, a bit $b \in \{0, 1\}$, and an adversary $\mathcal{A}$, we define the following security game $\mathsf{Exp}^{\mathsf{RABE-CD}}_{\mathcal{A}}(\lambda, b)$ between $\mathcal{A}$ and a challenger:

\begin{description}\setlength\itemsep{0.5em}
    \item[$\bullet$] \textbf{Setup phase:} The challenger samples the common reference string $\mathsf{crs} \leftarrow \mathsf{Setup}(1^{\lambda}, 1^{|\mathcal{U}|})$. It then initializes the internal state as follows: auxiliary input $\mathsf{aux} \leftarrow \perp$, master public key $\mathsf{mpk} \leftarrow \perp$, and counter $\mathsf{ctr} \leftarrow 0$ to track the number of honest key registration queries. It also initializes empty sets $C \leftarrow \emptyset, H \leftarrow \emptyset$ to record corrupted and honest public keys, respectively, and an empty dictionary $D \leftarrow \emptyset$ to map public keys to their associated attribute sets. For notational convenience, if $\mathsf{pk} \notin D$, we define $D[\mathsf{pk}] :=\emptyset$. Finally, the challenger sends $\mathsf{crs}$ to the adversary $\mathcal{A}$.

    \item[$\bullet$] \textbf{Query phase:} The adversary $\mathcal{A}$ can issue the following queries: \vspace{0.2cm}

    \begin{description}\setlength\itemsep{0.5em}
        \item[$-$] \textbf{Register corrupted key query:} $\mathcal{A}$ submits a public key $\mathsf{pk}$ along with a set of attributes $S \subseteq \mathcal{U}$. The challenger then executes
        \begin{align*}
            &(\mathsf{mpk}', \mathsf{aux}') \leftarrow\mathsf{RegPK}(\mathsf{crs},\mathsf{aux},\mathsf{pk},S)
        \end{align*}
        and updates the following
        \begin{align*}
            &\mathsf{mpk} \leftarrow \mathsf{mpk}',~C \leftarrow C \cup \{\mathsf{pk}\}\\
            &\mathsf{aux} \leftarrow \mathsf{aux}',~D[\mathsf{pk}] \leftarrow D[\mathsf{pk}] \cup \{S\}.
        \end{align*}
        Finally, the challenger replies to $\mathcal{A}$ with $(\mathsf{mpk}', \mathsf{aux}')$.

        \item[$-$] \textbf{Register honest key query:} In an honest-key-registration query, the adversary specifies a set of attributes $S \subseteq \mathcal{U}$. The challenger increments the counter $\mathsf{ctr} \leftarrow \mathsf{ctr} + 1$, samples a key pair $(\mathsf{pk}_{\mathsf{ctr}}, \mathsf{sk}_{\mathsf{ctr}}) \leftarrow \mathsf{KeyGen}(\mathsf{crs}, \mathsf{aux})$, and registers it by computing $(\mathsf{mpk}', \mathsf{aux}')$ $ \leftarrow$ $\mathsf{RegPK}(\mathsf{crs},$ $ \mathsf{aux},$ $\mathsf{pk}_{\mathsf{ctr}}, S)$. The challenger then updates its state as follows:
        \begin{align*}
            &\mathsf{mpk} \leftarrow \mathsf{mpk}',~H \leftarrow H \cup \{\mathsf{pk}_{\mathsf{ctr}}\},\\
            &\mathsf{aux} \leftarrow \mathsf{aux}',~D[\mathsf{pk}_{\mathsf{ctr}}] \leftarrow D[\mathsf{pk}_{\mathsf{ctr}}] \cup \{S\}.
        \end{align*}
        Finally, it replies to the adversary with $(\mathsf{ctr}, \mathsf{mpk}', \mathsf{aux}', \mathsf{pk}_{\mathsf{ctr}})$.

        \item[$-$] \textbf{Corrupt honest key query:} $\mathcal{A}$ specifies an index $1 \leq i \leq \mathsf{ctr}$. Let $(\mathsf{pk}_i, \mathsf{sk}_i)$ be the key pair generated during the $i$-th honest key query. The challenger updates its state by removing $\mathsf{pk}_i$ from $H$ and adding it to $C$:
        \begin{align*}
            &H \gets H \setminus \{\mathsf{pk}_i\}, ~C \gets C \cup \{\mathsf{pk}_i\}.
        \end{align*}
        It then returns $\mathsf{sk}_i$ to $\mathcal{A}$.
    \end{description}
    
    \item[$\bullet$] \textbf{Challenge phase:} In the challenge phase, $\mathcal{A}$ chooses two messages $\mu_0^*, \mu_1^* \in \mathcal{M}$ together with an access policy $P^* \in \mathcal{P}$. The challenger first verifies that 
    \[
        P^*(S) = 0 \quad \text{for all } S \in \{D[\mathsf{pk}] : \mathsf{pk} \in C\},
    \]
    ensuring that no corrupted key is authorized under $P^*$. Subsequently, the challenger selects a random bit $b\in\{0,1\}$ and executes the encryption algorithm
    \[
        (\mathsf{vk}^*, \mathsf{ct}_b^*) \gets \mathsf{Encrypt}(\mathsf{mpk}, P^*, \mu_b^*),
    \]
    and returns $\mathsf{ct}_b^*$ to $\mathcal{A}$. %In the case of a publicly verifiable scheme, the challenger instead returns the pair $(\mathsf{vk}^*, \mathsf{ct}_b^*)$.
    
    \item[$\bullet$] \textbf{Deletion phase:} At some point, the adversary $\mathcal{A}$ produces a deletion certificate $\mathsf{cert}$ and submits it to the challenger. The challenger verifies its validity by computing
    \[
        \mathsf{valid} \gets \mathsf{Verify}(\mathsf{vk}^*, \mathsf{cert}).
    \]
    If $\mathsf{valid} = 0$, the challenger aborts the experiment and outputs $\perp$.
    
    If $\mathsf{valid} = 1$, the challenger discloses the following information:
    \begin{description}
        \item[$-$] All honest secret keys $\{\mathsf{sk}_i : \mathsf{pk}_i \in H\},$
        \item[$-$] All helper keys generated via the update algorithm $$\{\mathsf{hsk}_i :\mathsf{hsk}_i \gets \mathsf{Update}(\mathsf{crs},\mathsf{aux},\mathsf{pk}_i),~ \mathsf{pk}_i \in H\}.$$
    \end{description}
    \item[$\bullet$] \textbf{Output phase:} The adversary outputs a bit $b' \in \{0,1\}$.
\end{description}

\noindent We say that $\prod^{\mathsf{RABE}}_{\textsf{CD}}$ is secure if for all efficient and admissible \textsf{QPT} adversaries $\mathcal{A}$, there exists a negligible function $\mathsf{negl}$ such that for all $\lambda \in \mathbb{N}$
\[
\left| \Pr\left[\mathsf{Exp}^{\mathsf{RABE-CD}}_{ \mathcal{A}}(\lambda, 0) = 1\right] - \Pr\left[\mathsf{Exp}^{\mathsf{RABE-CD}}_{\mathcal{A}}(\lambda, 1) = 1\right] \right| \leq \mathsf{negl}(\lambda).
\]

%---------------------------------






